mmGAT: Pose Estimation by Graph Attention with Mutual Features from mmWave Radar Point Cloud

Pose estimation and human action recognition (HAR) are pivotal technologies spanning various domains. While the image-based pose estimation and HAR are widely admired for their superior performance, they lack in privacy protection and suboptimal performance in low-light and dark environments. This paper exploits the capabilities of millimeter-wave (mmWave) radar technology for human pose estimation by processing radar data with Graph Neural Network (GNN) architecture, coupled with the attention mechanism. Our goal is to capture the finer details of the radar point cloud to improve the pose estimation performance. To this end, we present a unique feature extraction technique that exploits the full potential of the GNN processing method for pose estimation. Our model mmGAT demonstrates remarkable performance on two publicly available benchmark mmWave datasets and establishes new state of the art results in most scenarios in terms of human pose estimation. Our approach achieves a noteworthy reduction of pose estimation mean per joint position error (MPJPE) by 35.6% and PA-MPJPE by 14.1% from the current state of the art benchmark within this domain.

==> sections/actionformer.tex <==
---Experimental result section---

Apart from the pose estimation, mRI paper \cite{b2} also analyzed the quality of pose estimation by using the predicted poses to train ActionFormer \cite{b29} model. ActionFormer is a sequential action localization model. mRI data set already provided 12 action labels in P1 and 10 action labels in P2. According to \cite{b2}, they trained a supervised action localization model by feeding it the predicted poses and using the action labels as ground truth. We took similar approach and used ActionFormer model to evaluate the action localization performance from the predicted pose by mmGAT model.

To train ActionFormer, we used only S2P1 and S2P2 combinations of mRI radar data. We trained the pose estimation mmGAT model and then predicted continuous poses for all frames for all subjects for both training and test data set. We used the same split for training and evaluation of ActionFormer. We trained the ActionFormer model from scratch with the predicted poses from training set and then evaluated model performance with the predicted poses from test set.

The ActionFormer model accepts consistent feature vectors for each frame. To prepare that, we flattened the predicted 3D pose from mmGAT and used it as the feature vector for the corresponding frame. Thus created feature vectors for all frames of a subject.

The evaluation metric is mean average precision (mAP). Since the task is action localization, mAP was calculated by checking the detection segment’s intersection with ground truth temporal segment of an action and a temporal Intersection over Union (tIoU) was calculated and correct detection was decided by a threshold. We reported our results at tIoU of 0.5 at 2 Hz sampling frequency. We utilized open sourced training and evaluation scripts provided by ActionFormer authors \cite{b29}.


---- results analysis -----

Next we move on to the results from ActionFormer for human action localization task from the predicted 3D keypoints. We used two protocols from subject wise data splitting same as the reported scenarios in \cite{b2}. The results are described below. The scores are mAP and is a percentage without any specific unit.

\subfile{../tables/actionformer-results}


---- abstract ----

and action localization

keywords- actionformer, action localization

==> sections/references.tex <==
\section{References}

\begin{thebibliography}{00}

\bibitem{b1} An, Sizhe, and Umit Y. Ogras. "Mars: mmwave-based assistive rehabilitation system for smart healthcare." ACM Transactions on Embedded Computing Systems (TECS) 20.5s (2021): 1-22.
\bibitem{b2} An, Sizhe, Yin Li, and Umit Ogras. "mri: Multi-modal 3d human pose estimation dataset using mmwave, rgb-d, and inertial sensors." Advances in Neural Information Processing Systems 35 (2022): 27414-27426.
\bibitem{b3} Singh, Akash Deep, et al. "Radhar: Human activity recognition from point clouds generated through a millimeter-wave radar." Proceedings of the 3rd ACM Workshop on Millimeter-wave Networks and Sensing Systems. 2019.
\bibitem{b4} An, Sizhe, and Umit Y. Ogras. "Fast and scalable human pose estimation using mmwave point cloud." Proceedings of the 59th ACM/IEEE Design Automation Conference. 2022.
\bibitem{b5} Okamoto, Yoshihisa, and Tomoaki Ohtsuki. "Human activity classification and localization using bistatic three frequency CW radar." 2013 IEEE International Conference on Communications (ICC). IEEE, 2013.
\bibitem{b6} Yu, Cong, et al. "Fast 3D Human Pose Estimation Using RF Signals." ICASSP 2023-2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP). IEEE, 2023.
\bibitem{b7} Ishizaka, Shuzo, Kohei Yamamoto, and Tomoaki Ohtsuki. "Non-contact blood pressure measurement using doppler radar based on waveform analysis by LSTM." ICC 2021-IEEE International Conference on Communications. IEEE, 2021.
\bibitem{b8} Takabatake, Wataru, et al. "FMCW radar-based anomaly detection in toilet by supervised machine learning classifier." 2019 IEEE Global Communications Conference (GLOBECOM). IEEE, 2019.
\bibitem{b9} Hong, Jihoon, Shoichiro Tomii, and Tomoaki Ohtsuki. "Cooperative fall detection using Doppler radar and array sensor." 2013 IEEE 24th Annual International Symposium on Personal, Indoor, and Mobile Radio Communications (PIMRC). IEEE, 2013.
\bibitem{b10} Yamamoto, Kohei, Kentaroh Toyoda, and Tomoaki Ohtsuki. "CNN-based respiration rate estimation in indoor environments via MIMO FMCW radar." 2019 IEEE Global Communications Conference (GLOBECOM). IEEE, 2019.
\bibitem{b11} Ye, Chen, Kentaroh Toyoda, and Tomoaki Ohtsuki. "Robust heartbeat detection with Doppler radar based on stochastic gradient approach." 2018 IEEE International Conference on Communications (ICC). IEEE, 2018.
\bibitem{b12} Mogi, Eriko, and Tomoaki Ohtsuki. "Heartbeat detection with Doppler radar based on spectrogram." 2017 IEEE International Conference on Communications (ICC). IEEE, 2017.
\bibitem{b13} Ohtsuki, Tomoaki, and Eriko Mogi. "Heartbeat detection with Doppler radar based on estimation of average RR interval using Viterbi algorithm." 2016 IEEE 27th Annual International Symposium on Personal, Indoor, and Mobile Radio Communications (PIMRC). IEEE, 2016.
\bibitem{b14} Tomii, Shoichiro, and Tomoaki Ohtsuki. "Heartbeat detection by using Doppler radar with wavelet transform based on scale factor learning." 2015 IEEE International Conference on Communications (ICC). IEEE, 2015.
\bibitem{b15} Bouazizi, Mondher, Kohei Yamamoto, and Tomoaki Ohtsuki. "Heartbeat Detection Using 3D Lidar and MIMO Doppler Radar." ICC 2022-IEEE International Conference on Communications. IEEE, 2022.
\bibitem{b16} Yamamoto, Kohei, Koji Endo, and Tomoaki Ohtsuki. "Remote sensing of heartbeat based on space diversity using MIMO FMCW radar." 2021 IEEE Global Communications Conference (GLOBECOM). IEEE, 2021.
\bibitem{b17} Ye, Chen, Kentaroh Toyoda, and Tomoaki Ohtsuki. "A stochastic gradient approach for robust heartbeat detection with Doppler radar using time-window-variation technique." IEEE Transactions on Biomedical Engineering 66.6 (2018): 1730-1741.
\bibitem{b18} Yu, Danyuan, Mondher Bouazizi, and Tomoaki Ohtsuki. "A GAN-Based Data Augmentation Approach to Improve Heart Rate Range Classification via Doppler Radar." IEICE Technical Report; IEICE Tech. Rep. 123.110 (2023): 46-51.
\bibitem{b19} Xiong, Zhaoping, et al. "Pushing the boundaries of molecular representation for drug discovery with the graph attention mechanism." Journal of medicinal chemistry 63.16 (2019): 8749-8760.
\bibitem{b20} Jiang, Dejun, et al. "Could graph neural networks learn better molecular representation for drug discovery? A comparison study of descriptor-based and graph-based models." Journal of cheminformatics 13.1 (2021): 1-23.
\bibitem{b21} Xiong, Jiacheng, et al. "Graph neural networks for automated de novo drug design." Drug Discovery Today 26.6 (2021): 1382-1393.
\bibitem{b22} Strokach, Alexey, et al. "Fast and flexible protein design using deep graph neural networks." Cell systems 11.4 (2020): 402-411.
\bibitem{b23} Yin, Ruiping, et al. "A deeper graph neural network for recommender systems." Knowledge-Based Systems 185 (2019): 105020.
\bibitem{b24} Luna, Elena, et al. "Graph Neural Networks for Cross-Camera Data Association." IEEE Transactions on Circuits and Systems for Video Technology 33.2 (2022): 589-601.
\bibitem{b25} Veličković, Petar, et al. "Graph attention networks." arXiv preprint arXiv:1710.10903 (2017).
\bibitem{b26} Arjovsky, Martin, Soumith Chintala, and Léon Bottou. "Wasserstein generative adversarial networks." International conference on machine learning. PMLR, 2017.
\bibitem{b27} Wu, Jiacheng, Han Cui, and Naim Dahnoun. "A voxelization algorithm for reconstructing MmWave radar point cloud and an application on posture classification for low energy consumption platform." Sustainability 15.4 (2023): 3342.
\bibitem{b28} Lee, Shih-Po, et al. "Hupr: A benchmark for human pose estimation using millimeter wave radar." Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision. 2023.
\bibitem{b29} Cao, Zhongping, et al. "A Joint Global–Local Network for Human Pose Estimation with Millimeter Wave Radar." IEEE Internet of Things Journal 10.1 (2022): 434-446.
\bibitem{b30} Ross, Amy. "Procrustes analysis." Course report, Department of Computer Science and Engineering, University of South Carolina 26 (2004): 1-8.
\bibitem{b31} Rumelhart, David E., Geoffrey E. Hinton, and Ronald J. Williams. "Learning internal representations by error propagation." (1985).
\bibitem{b32} Kingma, Diederik P., and Jimmy Ba. "Adam: A method for stochastic optimization." arXiv preprint arXiv:1412.6980 (2014).
\bibitem{b33} Xie, Chunyang, et al. "Accurate Human Pose Estimation using RF Signals." 2022 IEEE 24th International Workshop on Multimedia Signal Processing (MMSP). IEEE, 2022.
\bibitem{b34} Zhong, Jinxiao, Liangnian Jin, and Ran Wang. "Point‐convolution‐based human skeletal pose estimation on millimetre wave frequency modulated continuous wave multiple‐input multiple‐output radar." IET Biometrics 11.4 (2022): 333-342.
\bibitem{b35} Sengupta, Arindam, et al. "mm-Pose: Real-time human skeletal posture estimation using mmWave radars and CNNs." IEEE Sensors Journal 20.17 (2020): 10032-10044.
\bibitem{b36} Hochreiter, Sepp, and Jürgen Schmidhuber. "Long short-term memory." Neural computation 9.8 (1997): 1735-1780.
\bibitem{b37} Nair, Vinod, and Geoffrey E. Hinton. "Rectified linear units improve restricted boltzmann machines." Proceedings of the 27th international conference on machine learning (ICML-10). 2010.
\bibitem{b38} Sengupta, Arindam, and Siyang Cao. "mmpose-nlp: A natural language processing approach to precise skeletal pose estimation using mmwave radars." IEEE Transactions on Neural Networks and Learning Systems (2022).
\bibitem{b39} Gong, Peixian, Chunyu Wang, and Lihua Zhang. "Mmpoint-gnn: Graph neural network with dynamic edges for human activity recognition through a millimeter-wave radar." 2021 International Joint Conference on Neural Networks (IJCNN). IEEE, 2021.
\bibitem{b40} Sutskever, Ilya, Oriol Vinyals, and Quoc V. Le. "Sequence to sequence learning with neural networks." Advances in neural information processing systems 27 (2014).

\end{thebibliography}

==> tables/actionformer-results.tex <==
\begin{table}[htbp]
\begin{center}
\caption{ActionFormer \cite{b29} activity localization results (in mAP with tIOU threshold of 0.5)}
\begin{tabular}{|c|c|c|}
\hline
Model & Protocol S2-P1 & Protocol S2-P2 \\
\hline
mRI paper & 98.22 & 99.00 \\
GNN model & 92.50 & 82.20 \\
\hline
\end{tabular}
\end{center}
\end{table}
